Faster Deep Reinforcement Learning with Slower Online Network

Deep reinforcement learning algorithms often use two networks for value function optimization: an online network, and a target network that tracks the online network with some delay. Using two separate networks enables the agent to hedge against issues that arise when performing bootstrapping. In this paper we endow two popular deep reinforcement learning algorithms, namely DQN and Rainbow, with updates that incentivize the online network to remain in the proximity of the target network. This improves the robustness of deep reinforcement learning in presence of noisy updates. The resultant agents, called DQN Pro and Rainbow Pro, exhibit significant performance improvements over their original counterparts on the Atari benchmark demonstrating the effectiveness of this simple idea in deep reinforcement learning. The code for our paper is available here: Github.com/amazon-research/fast-rl-with-slow-updates.

==> PI for Deep Reinforcement Learning (Neurips 2022)/abstract.tex <==
\begin{abstract}
Deep reinforcement learning algorithms often use two networks for value function optimization: an online network, and a target network that tracks the online network with some delay. Using two separate networks enables the agent to hedge against issues that arise when performing bootstrapping. In this paper we endow two popular deep reinforcement learning algorithms, namely DQN and Rainbow, with updates that incentivize the online network to remain in the proximity of the target network. This improves the robustness of deep reinforcement learning in presence of noisy updates. The resultant agents, called DQN Pro and Rainbow Pro, exhibit significant performance improvements over their original counterparts on the Atari benchmark demonstrating the effectiveness of this simple idea in deep reinforcement learning. The code for our paper is available here: Github.com/amazon-research/fast-rl-with-slow-updates.
\end{abstract}

==> PI for Deep Reinforcement Learning (Neurips 2022)/acknowledgement.tex <==
\section{Acknowledgment}
We thank Lihong Li, Pratik Chaudhari, and Shoham Sabach for their valuable insights in different stages of this work.

==> PI for Deep Reinforcement Learning (Neurips 2022)/background.tex <==
\section{Background and Notation}
RL is the study of the interaction between an environment and an agent that learns to maximize reward through experience. The Markov Decision Process~\citep{PutermanMDP1994}, or MDP, is used to mathematically define the RL problem. An MDP is specified by the tuple $\langle \mathcal{S,A,R,P,\gamma}
\rangle$, where $\mathcal{S}$ is the set of states and
$\mathcal{A}$ is the set of actions. The functions $\mathcal{R:S\times A\rightarrow}\ \mathbb R$ and
$\mathcal{P:S\times A \times S\rightarrow}\ [0,1]$ denote the reward and transition dynamics of the
MDP. Finally, a discounting factor $\gamma$ is used to formalize the intuition that short-term rewards are more valuable than those received later. 

The goal in the RL problem is to learn a policy, a mapping from states to a probability distribution over actions, ${\pi:\mathcal{S}\rightarrow \mathcal{P}(\mathcal{A})}$, that obtains high sums of future discounted rewards. An important concept in RL is the state value
function. Formally, it denotes the expected discounted sum of future rewards when committing to a policy $\pi$ in a state $s$: $v^{\pi}(s)\myeq \E\big[\sum_{t=0}^{\infty}\gamma^{t} R_t\big |S_0=s, \pi \big]\ .$
We define the Bellman operator $\mathcal{T^{\pi}}$ as follows:
\begin{equation*}
\label{eq:Bellman}
\big[\mathcal{T^{\pi}}v\big](s):=\!\sum_{a\in\mathcal{A}}\pi(a\mid s)\big(\mathcal{R}(s,a)+\!\sum_{s'\in \mathcal{S}}\!\gamma\ \mathcal{P}(s,a,s') v(s')\big)\ ,
\end{equation*}
which we can write compactly as: $\mathcal{T}^{\pi}v \myeq R^{\pi} + \gamma P^{\pi} v\ ,$ 
where $\big[R^{\pi}\big](s)= \sum_{a\in\mathcal{A}}\pi(a| s)\mathcal{R}(s,a)$ and $\big[P^{\pi} v\big](s)= \sum_{a\in\mathcal{A}}\pi(a\mid s)\sum_{s'\in \mathcal{S}}\!\mathcal{P}(s,a,s') v(s')$. We also denote:
 $(\mathcal{T}^{\pi})^{n}v\myeq\underbrace{\mathcal{T}^{\pi}\cdots\mathcal{T}^{\pi}}_{n\ \textrm{compositions}}v \ .$ Notice that $v^{\pi}$ is the unique fixed-point of $(\mathcal{T}^{\pi})^n$ for all natural numbers $n$, meaning that $ v^{\pi}=(\mathcal{T}^{\pi})^n v^{\pi}\ $, for all $n$. Define $v^{\star}$ as the optimal value of a state, namely: ${v^{\star}(s)\myeq \max_{\pi} v^{\pi}(s)} $, and $\pi^{\star}$ as a policy that achieves $v^{\star}(s)$ for all states. We define the Bellman Optimality Operator $\mathcal{T^{\star}}$:
\begin{equation*}
\label{eq:Bellman_Optimality}
\big[\mathcal{T^{\star}}v\big](s):=\!\max_{a\in\mathcal{A}}\mathcal{R}(s,a)+\!\sum_{s'\in \mathcal{S}}\!\gamma\ \mathcal{P}(s,a,s') v(s')\ ,
\end{equation*}
whose fixed point is $v^{\star}$. These operators are at the heart of many planning and RL algorithms including Value Iteration~\citep{bellamn1957} and Policy Iteration~\citep{howard1960dynamic}.

==> PI for Deep Reinforcement Learning (Neurips 2022)/commands.tex <==
\newcommand{\prox}[2]{\textrm{prox}_{#1}(#2)}
\newcommand{\proxNoParanthesis}[1]{\textrm{prox}_{#1}}
\newcommand{\norm}[3]{\left\lVert#1\right\rVert_{#2}^{#3}}
\newcommand{\empiricalExpectation}[1]{\widehat{\text E}_{#1}}
\newcommand{\expectation}[1]{\textup E_{#1}}
\newcommand{\dotProduct}[2]{\langle #1,#2 \rangle}
\newcommand{\variance}[0]{\textbf{Var}}

\newcommand{\algname}{DQNPro}
\newcommand{\algfullname}{Deep Q-Network with Proximal Iteration}
\newcommand{\E}{\mathbb{E}}
\newcommand\myeq{\vcentcolon=}

==> PI for Deep Reinforcement Learning (Neurips 2022)/conclusion_and_future_work.tex <==
\section{Conclusion and Future work}
We showed a clear advantage for using proximal terms to perform slower but more effective updates in approximate planning and reinforcement learning. Our results demonstrated that proximal updates lead to more robustness with respect to noise. Several improvements to proximal methods exist, such as the acceleration algorithm~\citep{nesterov,li2015accelerated}, as well as using other proximal terms~\citep{proximal_signal_processing}, which we leave for future work.
\label{s:conc}

==> PI for Deep Reinforcement Learning (Neurips 2022)/experiments.tex <==
\section{Experiments}\label{sec:experiment}

In this section, we empirically investigate the effectiveness of proximal updates in planning and reinforcement-learning algorithms. We begin by conducting experiments with PMPI in the context of approximate planning, and then move to large-scale RL experiments in Atari.

\subsection{PMPI Experiments}
We now focus on understanding the empirical impact of adding the proximal term on the performance of approximate PMPI. To this end, we use the pair of update equations:
\begin{eqnarray*}
\pi_{k} &\leftarrow& \mathcal{G} v_{k-1}\ ,\\
v_{k} &\leftarrow& (1-\beta)\big((\mathcal{T}^{\pi_{k}})^{n} v_{k-1} + \epsilon_{k}\big) +\beta v_{k-1}\ .
\end{eqnarray*}
For this experiment, we chose the toy $8\times8$ Frozen Lake environment from Open AI Gym~\citep{openaiGym}, where the transition and reward model of the environment is available to the planner. Using a small environment allows us to understand the impact of the proximal term in the simplest and most clear setting. Note also that we arranged the experiment so that the policy greedification step $\mathcal{G} v_{k-1}\ \forall k$ is error-free, so we can solely focus on the interplay between the proximal term and the error caused by imperfect policy evaluation.

We applied 100 iterations of PMPI, then measured the quality of the resultant policy $\pi\myeq\pi_{100}$ as defined by the distance between its true value and that of the optimal policy, namely $\norm{V^{\star} - V^{\pi}}{\infty}{}$. We repeated the experiment with different magnitudes of error, as well as different values of the $\beta$ parameter.
% zzz MLL: What's a magnitude of error? The previous paragraph says updates are error free (?).

\begin{figure}[ht]
\vspace*{-0.7em}
\centering\captionsetup[subfigure]{justification=centering}
\begin{subfigure}{0.45\textwidth}
\centering 
\includegraphics[width=\textwidth]{MPI/n=1.pdf} 
\end{subfigure}
\begin{subfigure}{ 0.45\textwidth} 
\centering 
\includegraphics[width=\textwidth]{MPI/n=3.pdf} 
\end{subfigure}
\caption{ Performance of approximate PMPI has a U-shaped dependence on the parameter $\beta=\frac{1}{1+c}$. Results are averaged over 30 random seeds with $n=1$ \textbf{(left)} and $n=3$ \textbf{(right)}.}
\label{fig:MPI} 
\end{figure}

From Figure \ref{fig:MPI}, it is clear that the final performance exhibits a U-shape with respect to the parameter $\beta$. It is also noticable that the best-performing $\beta$ is shifting to the right side (larger values) as we increase the magnitude of noise. This trend makes sense, and is consistent with what is predicted by Theorem~2: As the noise level rises, we have more incentive to use larger (but not too large) $\beta$ values to hedge against it.
% , but we may slow down the progress too much by choosing an extremely large $\beta$, therefore a larger (but an intermediate) value of $\beta$ works best.

\subsection{Atari Experiments}

In this section, we evaluate the proximal (or Pro) agents relative to their original DQN-style counterparts on the Atari benchmark~\citep{bellemare_atari}, and show that endowing the agent with the proximal term can lead into significant improvements in the interim as well as in the final performance. We next investigate the utility of our proposed proximal term through further experiments. Please see the Appendix for a complete description of our experimental pipeline.

\subsubsection{Setup}\label{sec:expsetup}

We used 55 Atari games~\citep{bellemare_atari} to conduct our experimental evaluations. Following \citet{MachadoAracde2017} and \citet{dopamine}, we used sticky actions to inject stochasticity into the otherwise deterministic Atari emulator.

Our training and evaluation protocols and the hyper-parameter settings follow those of the Dopamine baseline~\citep{dopamine}. To report performance, we measured the undiscounted sum of rewards obtained by the learned policy during evaluation. We further report the learning curve for all experiments averaged across 5 random seeds. We reiterate that we used the exact same hyper-parameters for all agents to ensure a sound comparison. 
\begin{figure}[ht]
\vspace*{-0.7em}
\centering\captionsetup[subfigure]{justification=centering}
\begin{subfigure}{0.425\textwidth}
\centering 
\includegraphics[width=\textwidth]{8_hyper_parameter_search/radar_dqn.png} 
\end{subfigure}
\begin{subfigure}{ 0.425\textwidth} 
\centering 
\includegraphics[width=\textwidth]{8_hyper_parameter_search/radar_rainbow.png} 
\end{subfigure}
\caption{ A minimal hyper-parameter tuning for $\tilde c$ in DQN Pro \textbf{(left)} and Rainbow Pro \textbf{(right)}.}
\label{fig:hyper_parameter} 
\end{figure}

Our Pro agents have a single additional hyper-parameter $\tilde c$. We did a minimal random search on 6 games to tune $\tilde c$. Figure~\ref{fig:hyper_parameter} visualizes the performance of Pro agents as a function of $\tilde c$. In light of this result, we set $\tilde c = 0.2$ for DQN Pro and $\tilde c = 0.05$ for Rainbow Pro. We used these values of $\tilde c$ for all 55 games, and note that we performed no further hyper-parameter tuning at all.

\subsubsection{Results}\label{sec:results}
The first question is whether endowing the DQN agent with the proximal term can yield significant improvements over the original DQN.
\begin{figure*}[ht]
\centering
\captionsetup{}
\begin{subfigure}{1\linewidth} 
\centering 
\includegraphics[width=\textwidth]{1_main_comparison/pdqn_dqn.pdf} 
\end{subfigure} 
\begin{subfigure}{1\linewidth} 
\centering 
\includegraphics[width=\textwidth]{1_main_comparison/rainbow_vs_rainbowPro.pdf}
\end{subfigure}
\caption{
Final gain for DQN Pro over DQN \textbf{(top)}, and Rainbow Pro over Rainbow \textbf{(bottom)}, averaged over 5 seeds. DQN Pro and Rainbow Pro significantly outperform their original counterparts.}
\label{fig:final_performance_atari}
\end{figure*} 
Figure \ref{fig:final_performance_atari} (top) shows a comparison between DQN and DQN Pro in terms of the final performance. In particular, following standard practice~\citep{wang2016dueling, iqn, van2019using}, for each game we compute:
$$
\frac{\textrm{Score}_{\textrm{DQN Pro}} - \textrm{Score}_{\textrm{DQN}} }{ \max(\textrm{Score}_{\textrm{DQN}},\textrm{Score}_{\textrm{Human}}) - \textrm{Score}_{\textrm{Random}} }
\ .$$

Bars shown in red indicate the games in which we observed better final performance for DQN Pro relative to DQN, and bars in blue indicate the opposite. The height of a bar denotes the magnitude of this improvement for the corresponding benchmark; notice that the y-axis is scaled logarithmically. We took human and random scores from previous work~\citep{nair2015massively, iqn}. It is clear that DQN Pro dramatically improves upon DQN. We defer to the Appendix for full learning curves on all games tested. 

Can we fruitfully combine the proximal term with some of the existing algorithmic improvements in DQN? To answer this question, we build on the Rainbow algorithm of~\citet{rainbow} who successfully combined numerous important algorithmic ideas in the value-based RL literature. We present this result in Figure \ref{fig:final_performance_atari} (bottom). Observe that the overall trend is for Rainbow Pro to yield large performance improvements over Rainbow.

Additionally, we measured the performance of our agents relative to human players. To this end, and again following previous work~\citep{wang2016dueling, iqn, van2019using}, for each agent we compute the human-normalized score:
$$
\frac{\textrm{Score}_{\textrm{Agent}} - \textrm{Score}_{\textrm{Random}} }{ \textrm{Score}_{\textrm{Human}}- \textrm{Score}_{\textrm{Random}} } .
$$
In Figure~\ref{fig:main_learning_curve} (left), we show the median of this score for all agents, which~\citet{wang2016dueling} and~\citet{rainbow} argued is a sensible quantity to track. We also show per-game learning curves with standard error in the Appendix.

We make two key observations from this figure. First, the very basic DQN Pro agent is capable of achieving human-level performance (1.0 on the y-axis) after 120 million frames. Second, the Rainbow Pro agent achieves 220 percent human-normalized score after only 120 million frames.

\begin{figure}
  \begin{minipage}{0.55\textwidth}
    \includegraphics[width=\textwidth]{0_main_comparison_rainbow/median_learning_curves.pdf}
\end{minipage}
\hspace{2pt}
\begin{minipage}{0.375\textwidth}
\includegraphics[width=.5\textwidth]{3_norm_comparison/BeamRiderNoFrameskip-v0_norm_of_target_updates.png}%
\includegraphics[width=.5\textwidth]{3_norm_comparison/WizardOfWorNoFrameskip-v0_norm_of_target_updates.png} 
\includegraphics[width=.5\textwidth]{3_norm_comparison/GopherNoFrameskip-v0_norm_of_target_updates.png}%
\includegraphics[width=.5\textwidth]{3_norm_comparison/BoxingNoFrameskip-v0_norm_of_target_updates.png} 
\label{fig:effect_of_proximal} 
\end{minipage}
\caption{\textbf{(left)}: Human-normalized median performance for DQN, Rainbow, DQN Pro, and Rainbow Pro on 55 Atari games. Results are averaged over 5 independent seeds. Our agents, Rainbow Pro (yellow) and DQN Pro (red) outperform their original counterparts Rainbow (green) and DQN (blue). \textbf{(right)}: Using the proximal term reduces the magnitude of target network updates.} 
\label{fig:main_learning_curve}
\end{figure}
\subsubsection{Additional Experiments}
Our purpose in endowing the agent with the proximal term was to keep the online network in the vicinity of the target network, so it would be natural to ask if this desirable property can manifest itself in practice when using the proximal term. In Figure \ref{fig:main_learning_curve}, we answer this question affirmatively by plotting the magnitude of the update to the target network during synchronization. Notice that we periodically synchronize online and target networks, so the proximity of the online and target network should manifest itself in a low distance between two consecutive target networks. Indeed, the results demonstrate the success of the proximal term in terms of obtaining the desired proximity of online and target networks.


While using the proximal term leads to significant improvements, one may still wonder if the advantage of DQN Pro over DQN is merely stemming from a poorly-chosen \textit{period} hyper-parameter in the original DQN, as opposed to a truly more stable optimization in DQN Pro. To refute this hypothesis, we ran DQN with various settings of the \textit{period} hyper-parameter $\{2000, 4000, 8000, 12000\}$. This set included the default value of the hyper-parameter (8000) from the original paper~\citep{mnih2015human}, but also covered a wider set of settings.

Additionally, we tried an alternative update strategy for the target network, referred to as Polyak averaging, which was popularized in the context of continuous-action RL~\citep{ddpg}: $\theta \leftarrow \tau w + (1-\tau) \theta$. For this update strategy, too, we tried different settings of the $\tau$ hyper-parameter, namely $\{0.05, 0.005, 0.0005\}$, which includes the value $0.005$ used in numerous papers~\citep{ddpg,td3,rbfdqn}.
\begin{figure}
\begin{minipage}{0.425\textwidth}
\includegraphics[width=.5\textwidth]{2_target_network1/BeamRiderNoFrameskip-v0_target_network1.png}%
\includegraphics[width=.5\textwidth]{2_target_network1/WizardOfWorNoFrameskip-v0_target_network1.png}
\includegraphics[width=.5\textwidth]{2_target_network1/GopherNoFrameskip-v0_target_network1.png}%
\includegraphics[width=.5\textwidth]{2_target_network1/BoxingNoFrameskip-v0_target_network1.png}
\end{minipage}
\hspace{20pt}
\begin{minipage}{0.425\textwidth}
\includegraphics[width=.5\textwidth]{2_target_network2/BeamRiderNoFrameskip-v0_target_network2.png}%
\includegraphics[width=.5\textwidth]{2_target_network2/WizardOfWorNoFrameskip-v0_target_network2.png}
\includegraphics[width=.5\textwidth]{2_target_network2/GopherNoFrameskip-v0_target_network2.png}%
\includegraphics[width=.5\textwidth]{2_target_network2/BoxingNoFrameskip-v0_target_network2.png}
\end{minipage}
\caption{A comparison between DQN Pro and DQN with periodic \textbf{(left)} and Polyak \textbf{(right)} updates.}
\label{fig:target_network}
\end{figure}

Figure \ref{fig:target_network} presents a comparison between DQN Pro and DQN with periodic and Polyak target updates for various hyper-parameter settings of \textit{period} and $\tau$. It is clear that DQN Pro is consistently outperforming the two alternatives regardless of the specific values of \textit{period} and $\tau$, thus clearly demonstrating that the improvement is stemming from a more stable optimization procedure leading to a better interplay between the two networks.

Finally, an alternative approach to ensuring lower distance between the online and the target network is to anneal the step size based on the number of updates performed on the online network since the last online-target synchronization. In this case we performed this experiment in 4 games where we knew proximal updates provide improvements based on our DQN Pro versus DQN resulst in Figure~\ref{fig:final_performance_atari}. In this case we linearly decreased the step size from the original DQN learning rate $\alpha$ to $\alpha'\ll \alpha$ where we tuned $\alpha'$ using random search. Annealing indeed improves DQN, but DQN Pro outperforms the improved version of DQN. Our intuition is that Pro agents only perform small updates when the target network is far from the online network, but naively decaying the learning rate can harm progress when the two networks are in vicinity of each other.
\begin{figure}
\centering\captionsetup[subfigure]{justification=centering,skip=0pt}
\begin{subfigure}[t]{0.24\textwidth} 
\centering 
\includegraphics[width=\textwidth]{12_additional/results/NameThisGameNoFrameskip-v0_learning_curves_4_domains.png} 
\label{fig:NameThisGameNoFrameskip-v0_learning_curves_4_domains.png} 
\end{subfigure}% 
~ 
\begin{subfigure}[t]{ 0.24\textwidth} 
\centering 
\includegraphics[width=\textwidth]{12_additional/results/ZaxxonNoFrameskip-v0_learning_curves_4_domains.png} 
\label{fig:ZaxxonNoFrameskip-v0_learning_curves_4_domains.png} 
\end{subfigure}% 
~ 
\begin{subfigure}[t]{ 0.24\textwidth} 
\centering 
\includegraphics[width=\textwidth]{12_additional/results/BattleZoneNoFrameskip-v0_learning_curves_4_domains.png} 
\label{fig:BattleZoneNoFrameskip-v0_learning_curves_4_domains.png} 
\end{subfigure}% 
~ 
\begin{subfigure}[t]{ 0.24\textwidth} 
\centering 
\includegraphics[width=\textwidth]{12_additional/results/AssaultNoFrameskip-v0_learning_curves_4_domains.png} 
\label{fig:AssaultNoFrameskip-v0_learning_curves_4_domains.png} 
\end{subfigure}% 
\vspace{-.5cm}
\caption{Learning-rate decay does not bridge the gap between DQN and DQN Pro.} 
% zzz accept on the problem where DQN was already winning, right? -MLL
% of the 6, 4 where DQNPro was winning and 2 where DQN was winning
\label{fig:rebut} 
\end{figure} 

\section{Discussion}
In our experience using proximal updates in the parameter space were far superior than proximal updates in the value space. We believe this is because the parameter-space definition can enforce the proximity globally, while in the value space one can only hope to obtain proximity locally and on a batch of samples. One may hope to use natural gradients to enforce value-space proximity in a more principled way, but doing so usually requires significantly more computational resources~\cite{knight2018natural}. This is in contrast to our proximal updates which add negligible computational cost in the simple form of taking a dimension-wise weighted average of two weight vectors.

In addition, for a smooth (Lipschitz) $Q$ function, performing parameter-space regularization guarantees function-space regularization. Concretely: $\forall s, \forall a \ |Q(s,a;\theta)-Q(s,a;\theta')|\leq L||\theta-\theta'||\ , $ where $L$ is the Lipschitz constant of $Q$. Moreover, deep networks are Lipschitz~\citep{neyshabur2015norm, asadi2018lipschitz}, because they are constructed using compositions of Lipschitz functions (such as ReLU, convolutions, etc) and that composition of Lipschitz functions is Lipschitz. So performing value-space updates may be an overkill. Lipschitz property of deep networks has successfully been leveraged in other contexts, such as in generative adversarial training~\cite{arjovsky2017wasserstein}.

A key selling point of our result is simplicity, because simple results are easy to understand, implement, and reproduce. We obtained significant performance improvements by adding just a few lines of codes to the publicly available implementations of DQN and Rainbow~\cite{dopamine}.

==> PI for Deep Reinforcement Learning (Neurips 2022)/introduction.tex <==
\section{Introduction}
An important competency of reinforcement-learning (RL) agents is learning in environments with large state spaces like those found in robotics~\citep{kober_robotics}, dialog systems~\citep{williams2017hybrid}, and games~\citep{td_gammon, silver2017mastering}. Recent breakthroughs in deep RL have demonstrated that simple approaches such as Q-learning~\citep{q_learning} can surpass human-level performance in challenging environments when equipped with deep neural networks for function approximation~\citep{mnih2015human}.

Two components of a gradient-based deep RL agent are its objective function and optimization procedure. The optimization procedure takes estimates of the gradient of the objective with respect to network parameters and updates the parameters accordingly. In DQN~\citep{mnih2015human}, for example, the objective function is the empirical expectation of the temporal difference (TD) error~\citep{sutton_td} on a buffered set of environmental interactions~\citep{lin1992self}, and variants of stochastic gradient descent are employed to best minimize this objective function.

A fundamental difficulty in this context stems from the use of bootstrapping. Here, bootstrapping refers to the dependence of the target of updates on the parameters of the neural network, which is itself continuously updated during training. Employing bootstrapping in RL stands in contrast to supervised-learning techniques and Monte-Carlo RL~\citep{rl_book}, where the target of our gradient updates does not depend on the parameters of the neural network. 

\citet{mnih2015human} proposed a simple approach to hedging against issues that arise when using bootstrapping, namely to use a \textit{target network} in value-function optimization. The target network is updated periodically, and tracks the online network with some delay. While this modification constituted a major step towards combating misbehavior in Q-learning~\citep{target_based_TD, kim2019deepmellow, zhang_breaking_deadly_triad}, optimization instability is still prevalent~\citep{van_hasselt_deadly_triad}.

Our primary contribution is to endow DQN and Rainbow~\citep{rainbow} with a term that ensures the parameters of the online-network component remain in the proximity of the parameters of the target network. Our theoretical and empirical results show that our simple proximal updates can remarkably increase robustness to noise without incurring additional computational or memory costs. In particular, we present comprehensive experiments on the Atari benchmark~\citep{bellemare_atari} where proximal updates yield significant improvements, thus revealing the benefits of using this simple technique for deep RL.

==> PI for Deep Reinforcement Learning (Neurips 2022)/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> PI for Deep Reinforcement Learning (Neurips 2022)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}
\usepackage{mathtools}
% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> PI for Deep Reinforcement Learning (Neurips 2022)/proximal_bellman_operator.tex <==
\section{The Proximal Bellman Equation}
Define 

$$T_{\proxNoParanthesis{h}}(Q):=\proxNoParanthesis{h}\big(T(Q)\big).$$
We show that $Q^{*}$, defined as the fixed point of the original Bellman equation, $Q^{*}=TQ^{*}$ is also the fixed point of the proximal Bellman equation:
$$Q^{*}=\proxNoParanthesis{h}\big(T(Q^*)\big)\ ,$$
under zzz condition on $h$. This result demonstrates that, while adding the proximal term biases the interim solution towards those with small $h$, this bias will vanish as we converge to the fixed-point solution in light of the equivalence between the fixed points of $T$ and $T_{\proxNoParanthesis{h}}$. We prove this statement in the following Theorem:

\begin{theorem}
\label{thm:convergence_general}
Let $\mathcal{O}:\mathcal{V} \rightarrow \mathcal{V}$ be a contraction operating on the vector space $\mathcal{V}$. Let
\begin{align}
    \prox{f,V'}{V} \equiv \argmin_{\hat{V}} \left[ f(V, \hat{V}) + \norm{\hat{V} - V'}{2}{2} \right]
\end{align}

\textcolor{red}{$$ 
    \prox{f,V'}{V} \equiv \argmin_{\hat{V}} \left[ f(V', \hat{V}) + \norm{\hat{V} - V}{2}{2} \right]$$}
% \begin{align}
%     \prox{f,V'}{V} \equiv \argmin_{\hat{V}} \left[ f(\hat{V}, \hat{V}) + \norm{\hat{V} - V}{2}{2} \right]
% \end{align}

with $f:\mathcal{V} \times \mathcal{V} \rightarrow \mathbb{R}$ a convex function such that $\argmin_V f(V, V') = V'$. Then, the sequence $V_k$ given by

\begin{align}
    V_{k+1} = \prox{f,\mathcal{O}(V_k)}{\mathcal{O}(V_k)}
\end{align}

and any $V_0 \in \mathcal{V}$ converges to the fixed point of $\mathcal{O}$, denoted as $V^*$.

\end{theorem}

\begin{proof}
Define the operator

\begin{align}
    \mathcal{O}_{\textbf{prox}_{f,V'}}(V) = \prox{f,V'}{\mathcal{O}(V)} = (\textbf{prox}_{f,V'} \circ \mathcal{O}) (V).
\end{align}
Then, we can write the sequence $V_k$ as $V_{k+1} = (\textbf{prox}_{f,V_k} \circ \mathcal{O}) (V_k)$. Because the proximal operator is a non-expansion, and $\mathcal{O}$ is a contraction, the composition $\textbf{prox}_{f,V_k} \circ \mathcal{O}$ is also a contraction and therefore has a unique fixed point. We must therefore only show that $V^*$ is a fixed point of
\begin{align}
    \prox{f,V^*}{V} \equiv \argmin_{\hat{V}} \left[ f(V, \hat{V}) + \norm{\hat{V} - V^*}{2}{2} \right].
\end{align}

\textcolor{red}{$$ \prox{f,V^*}{V} \equiv \argmin_{\hat{V}} \left[ f(V^*, \hat{V}) + \norm{\hat{V} - V}{2}{2} \right]
$$}

\textcolor{red}{$$ = \argmin_{\hat{V}} \left[ f(V^*, \hat{V}) + \norm{\hat{V} - V}{2}{2} \right]
$$}

% \begin{align}
%     \prox{f,V^*}{V} \equiv \argmin_{\hat{V}} \left[ f(V, V^*) + \norm{\hat{V} - V}{2}{2} \right].
% \end{align}

But $V^*$ eliminates the second term and, by our assumption on $f(V)$, minimizes the first term. Therefore, $\prox{f,V^*}{V^*} = V^*$.

\end{proof}

Note that Theorem \ref{thm:convergence_general} is much more general and extends beyond applying an $L_2$ norm to the Bellman operator. It shows that the adding a proximal step can be applied to many RL operators without biasing the fixed point these algorithms converge to. Thus, for example, when applying the proximal step to linear function approximation of the Bellman operator {\bf a reference would be good}, we would still converge to the same projected fixed point of the Bellman operator onto the linear space, because projections maintain the contraction properties of operators. Furthermore, $f(V)$ does not necessarily have to be the $L_2$ norm (and doesn't even have to be a norm), opening the door to a variety of potential algorithms using different convex regularization functions. % zzz MLL: I'd move the more abstract Lemma 2 into supplementary material since the proof is SO similar to the first one and is mainly here for flag planting, it seems.

Notation-wise, we have

$$T_{\proxNoParanthesis{h}}(Q):=\proxNoParanthesis{h(\cdot;Q)}(Q)$$
i.e. when the argument of T and the second argument of $h$ are the same, we just drop it from $h$ for readability. also please always use $h$ as the letter that indicates a generic proximal function.

% We first show that the operator $T_{\prox{f}{V}}$ converges to the same fixed point as $T$, that is, both converge to the optimal value function $V^*$.

% \begin{lemma}
% \label{lemma:simple_convergence}
%     The operator $T_{\prox{f}{V}}$ is a contraction, with the same fixed point, $V^*$, as the Bellman operator, $T$. 
% \end{lemma}

% \begin{proof}
% The $T_{\prox{f}{V}}$ is a composition of the Bellman operator and the proximal operator. Because the Bellman operator is a contraction (CITE) and the proximal operator is a non-expansion \citep{beck_book}, their composition is also a contraction, and therefore has a unique fixed point. We therefore only need to show that $V^*$, the fixed point of $T$, is also a fixed point of $T_{\prox{f}{V}}$.

% At $V^*$, $T_{\prox{f}{V}}$ can be explicitly written as:

% \begin{align*}
%     T_{\prox{f}{V^*}}(V) \equiv \argmin_{\hat{V}} \left[ \norm{TV - \hat{V}}{2}{2} + \norm{V^*-\hat{V}}{2}{2} \right].
% \end{align*}

% % MLL: I'd make this point differently.
% Setting $\hat{V} = V^*$, makes the second term zero and also makes the first term zero because $V^*$ is a fixed point of $T$. The entire expression is necessarily non-negative, making $V^*$ a minimizer. Thus, $T_{\prox{f}{V^*}}(V^*) = V^*$; $V^*$ is a fixed point.

% % For $\hat{V} = V^*$, the first term vanishes because $V^*$ is a fixed point of T, and the second term vanishes trivially. The entire expression to be minimized by the operator is non-negative, and therefore minimized by $V^*$. Thus $T_{\prox{f}{V^*}}(V^*) = V^*$

% \end{proof}


==> PI for Deep Reinforcement Learning (Neurips 2022)/proximal_deep_q_network.tex <==
\section{Deep Q-Network with Proximal Updates}
We now endow DQN-style algorithms with proximal updates. Let $\langle s,a,r,s'\rangle$ denote a buffered tuple of interaction. Define the following objective function:
\begin{equation}\label{eq:td_error}
  h(\theta,w):=\empiricalExpectation{\langle s,a,r,s'\rangle}\Big[\big(r+\gamma \max_{a'} \widehat Q(s',a';\theta)- \widehat Q(s,a;w)\big)^2\Big]\  . 
\end{equation}

Our proximal update is defined as follows:
\begin{equation}
w_{t+1} \leftarrow \arg\min_{w} h(w_t,w)+\frac{1}{2\tilde c}\norm{w-w_{t}}{2}{2}\ . \label{eq:prox_for_deep_rl}
\end{equation}

This algorithm closely resembles the standard proximal-point algorithm~\citep{RockafellarProxPaper1976,prox_parikh_boyd} with the important caveat that the function $h$ is now taking two vectors as input. At each iteration, we hold the first input constant while optimizing over the second input. 

In the optimization literature, the proximal-point algorithm is well-studied in contexts where an analytical solution to (\ref{eq:prox_for_deep_rl}) is available. With deep learning no closed-form solution exists, so we approximately solve (\ref{eq:prox_for_deep_rl}) by taking a fixed number of descent steps using stochastic gradients. Specifically, starting each iteration with $w=w_t$, we perform multiple $w$ updates ${w \leftarrow  w -\alpha\big(\nabla_{2} h(w_t,w) + \frac{1}{\tilde c} (w-w_t)\big)}$. We end the iteration by setting $w_{t+1}\leftarrow w$.
To make a connection to standard deep RL, the online weights $w$ could be thought of as the weights we maintain in the interim to solve~(\ref{eq:prox_for_deep_rl}) due to lack of a closed-form solution. Also, what is commonly referred to as the target network could better be thought of as just the previous iterate in the above proximal-point algorithm.

Observe that the update can be written as: $w\leftarrow \big(1-(\alpha/\tilde c)\big) \cdot w +(\alpha/\tilde c) \cdot w_t -\alpha \nabla_{2} h(w_t,w) \  .
\label{eq:online_update_2}
$ Notice the intuitively appealing form: we first compute a convex combination of $w_t$ and $w$, based on the hyper-parameters $\alpha$ and $\tilde c$, then add the gradient term to arrive at the next iterate of $w$. If $w_t$ and $w$ are close, the convex combination is close to $w$ itself and so this DQN with proximal update ({\sl DQN Pro}) would behave similarly to the original DQN. However, when $w$ strays too far from $w_t$, taking the convex combination ensures that $w$ gravitates towards the previous iterate $w_t$. The gradient signal from minimizing the squared TD error~(\ref{eq:td_error}) should then be strong enough to cancel this default gravitation towards $w_t$. The update includes standard DQN as a special case when $\tilde c\rightarrow \infty$. The pseudo-code for DQN is presented in the Appendix. The difference between DQN and DQN Pro is minimal (shown in gray), and corresponds with a few lines of code in our implementation.

==> PI for Deep Reinforcement Learning (Neurips 2022)/proximal_operator.tex <==
\section{Proximal Operator [TODO merge ]}
\label{sec:proximal_operator}
Consider the following optimization problem:
\begin{equation}
    %\arg\min_w h(w)\ ,
    \min_w ~h(x;w)\ ,
    \label{eq:original_problem}
\end{equation}
%where $h$ could be any objective function such as a loss function for learning the Q-function in reinforcement learning, and $w$ denotes the parameters of the network we desire to learn. Suppose we have access to stochastic estimates of the gradient of the function $\nabla h$. Standard first-order optimization, such as stochastic gradient descent (SGD), can be employed to solve this optimization problem:
where $h$ is the objective function (e.g., standard temporal difference (TD) error in reinforcement learning~\ref{eq:td_error}), $w$ denotes the learnable parameters (e.g., the parameters of a Q-network), and $x$ is the input data (e.g., $\langle s, a, r, s' \rangle$). If $h$ is differentiable, then stochastic gradient descent (SGD), which proceeds as follows:
%$$w_{k+1}\leftarrow w_{k} -\alpha_{k} \nabla h(w_k)\ ,$$
\begin{equation}\label{eq:sgd}
w_{k}\leftarrow w_{k-1} -\alpha_{k} \nabla_w h(x;w_{k-1}), ~~~k=1,2,3,\dots
\end{equation}
could be used to solve the optimization problem~(\ref{eq:original_problem}). Here, $\alpha_k$ denotes the step size at iteration $k$, and $w_0$ is an arbitrary starting point.

While SGD is well-behaved asymptotically and under standard assumptions, it can perform recklessly in the interim, leading into a situation where the iterates get exponentially far from the %optimal
solution~\citep{BachNIPS2011, ryu_boyd_proximal}. This behavior can be particularly disruptive in the context of RL where sample efficiency is an important concern.

One simple and effective approach to stabilizing SGD is to augment the objective with a quadratic regularizer to ensure that the solution at each iteration stays in the vicinity of the previous ones:
%. This can be obtained by augmenting the objective as follows:
\begin{equation}
    w_{k} = \arg\min_w h(w) + \frac{1}{2c}\norm{w-w_{k-1}}{2}{2}\ .
    \label{eq:modified_problem}
\end{equation}
The quadratic term is basically a proximal term that ensures the next iterate $w_k$ will not stray too far from the previous iterate $w_{k-1}$. Having completed iteration $k$, we replace the previous iterate $w_{k-1}$ by its new value $w_k$ and then proceed to iteration $k+1$.
\iffalse 
To understand the behavior of this iterative process, called Proximal Iteration~\citep{prox_parikh_boyd, ryu_boyd_proximal}, we define the proximal operator:
\begin{equation}
    \prox{c, h}{w_k}:=\arg\min_{w}\ \frac{1}{c}\norm{w-w_{k-1}}{2}{2} +\ h(w)\ ,
\end{equation}
Proximal Iteration could be written as:
$$
w_{k}\leftarrow \prox{h}{w_{k-1}}\ ~~~k=1, 2, 3\dots
$$
From the Banach fixed-point theorem, we know that iteratively applying $\proxNoParanthesis{h}$ eventually converges to a unique fixed point provided that the operator is a contraction. \cite{bauschke2012firmly} have shown that, if the function $h$ is $\mu$-strongly convex, then the operator $\proxNoParanthesis{h}$ is indeed a contraction:
$$\norm{\prox{h}{w}-\prox{h}{w'}}{}{}\leq \frac{1}{1+\mu}\norm{w-w'}{}{}\ ,$$
and therefore iteratively applying the operator would guarantee convergence. 

What is the fixed-point of this operator? It is possible to show that it is the minimum of the function $h$, i.e., $\arg\min_{w} h(w)$, the minimum of problem~(\ref{eq:original_problem}), which we originally sought to solve~\citep{bauschke2011convex}. 

Therefore, the intuitive way of thinking about the Proximal Iteration algorithm, which is sometimes referred to as disappearing Tikhonov regularization~\citep{prox_parikh_boyd}, is as a principled way to bias the optimization path towards the previous iterate using the quadratic-norm penalty without altering the final answer. In other words, as Proximal Iteration makes progress, the previous iterate $w_{k-1}$ gets closer to $w^{\star}=\arg \min h(w)$ in light of the contraction property, therefore the contribution of the quadratic term vanishes to zero thus not biasing the asymptotic solution. The following remark sheds more light on the relationship between Proximal Iteration and trust-region algorithms:

[\textbf{Relationship between trust region and Proximal Iteration}]\label{rem:trust-region}
Define the trust-region problem as follows:
\begin{align*}\label{eq:trust_problem}
    %&\arg\min_w ~h(w)\\
    & \displaystyle{\min}_w ~h(w)\\
    &\text{s.t.}\ \norm{w-w_{k-1}}{2}{} \leq \rho\ , 
\end{align*}
\cite{prox_parikh_boyd} show that solving the above trust-region formulation is equivalent to a step of Proximal Iteration under appropriate choices of  $\rho$ (above) and $c$ (in prox). Therefore, iteratively applying the two formulations leads to the same solution. (See their Section~3.4 for more details.) %This interpretation provides \
%\todo[ "trust region formulation is equivalent to a step of Proximal" is not what they showed and I don't think so "a step of Proximal Iteration" is their result. they clearly showed proximal and trust region both get to the same solution with some combination of their hyper-params.... What I originally wrote provided a right version for their results: \cite{prox_parikh_boyd} shows that above trust region formulation and proximal problem~\eqqref{eq:modified_problem} are related and both methods can get to the same solutions for appropriate choices of their parameters (i.e $\rho$, $c$ ) (see section 3.4 in their paper for more details). Kavosh: one step of proximal iteration = one step of trust region, do both multiple times and you get the same answer.]
The second remark highlights the strength of Proximal Iteration relative to SGD:
[\textbf{The non-asymptotic advantage of Proximal Iteration over SGD}]\label{rem:non-asymptotic}
\fi
While the asymptotic performance of SGD and Proximal Iteration are analogous~\citep{ryu_boyd_proximal}, they may exhibit qualitatively different behavior in a non-asymptotic sense. More concretely, denote the stepsize of SGD and Proximal Iteration at iteration $k$ by $\alpha_k=\frac{C}{k}$, and $w^{\star}:=\arg\min_w h(w)$. For SGD, we have~\citep{bauschke2011convex}:
$$\expectation{}\big[\norm{w_k-w^{\star}}{2}{2}\big]\leq \mathcal{O}\left(\frac{\textrm{exp}(C^{2})}{k^{ C}} + \frac{1}{k}\right)\ .$$
The exponential dependence on $C$ can indeed manifest itself as \cite{ryu_boyd_proximal} demonstrate. In contrast, for Proximal Iteration we have~\citep{ryu_boyd_proximal}:
$$\expectation{}\big[\norm{w_k-w^{\star}}{2}{2}\big]\leq \norm{w_0-w^{\star}}{2}{2} +\sum_{i=1}^k \alpha_i\ .$$
While the iterates of SGD can get exponentially far from the optimal answer~\citep{BachNIPS2011, ryu_boyd_proximal}, Proximal Iteration is fairly well-behaved in the interim. This property is particularly valuable in the context of reinforcement learning where sample-efficiency, and not just the asymptotic performance, is of utmost importance.

\iffalse
In the context of a parameterized $Q$-function in RL, commonly used loss functions are not convex; however, several works have introduced convex loss via linear approximation. \citet{target_based_TD} have shown that in linear policy evaluation the loss function is convex in the weights. \citet{serrano2021logistic} introduced a convex loss function for control with linear approximation. These works demonstrate that many useful convex minimization objectives exist for RL.

In the case of deep RL, the loss function is not convex, and few convergence results exist for most state-of-the-art algorithms. Nevertheless, we follow standard practice and show that Proximal Iteration achieves significant empirical improvements when applied to standard deep RL algorithms. Furthermore, recent work provides convergence results for Proximal Iteration in specific non-convex cases, such as when $h(w)$ can be decomposed into a sum of a smooth non-convex function and non-smooth convex function~\citep{fukushima1981generalized, j2016proximal, li2018simple}. These recent results open the door for potential future developments toward proving convergence for Proximal Iterations in RL, which would further strengthen its theoretical grounding.
\fi

==> PI for Deep Reinforcement Learning (Neurips 2022)/related_work.tex <==
\section{Related Work}

The introduction of proximal operators could be traced back to the seminal work of~\citet{moreauhal-01867195,Moreau1965}, \citet{prox_first_work} and \citet{RockafellarProxPaper1976}, and the use of the proximal operators has since expanded into many areas of science such as signal processing~\citep{proximal_signal_processing}, statistics and machine learning~\citep{beck2009fast, prox_statistics, Reddi2015DoublyRC}, and convex optimization~\citep{prox_parikh_boyd, Bertsekas2011IncrementalPM, Bertsekas15cSrv}.

In the context of RL, \citet{proximal_rl_mahadevan} introduced a proximal theory for deriving convergent off-policy algorithms with linear function approximation. One intriguing characteristic of their work is that they perform updates in primal-dual space, a property that was leveraged in sample complexity analysis~\citep{prox_finite_liu} for the proximal counterparts of the gradient temporal-difference algorithm~\citep{gtd}. Proximal operators also have appeared in the deep RL literature. For instance, \citet{fakoor2020metaqlearning} used proximal operators for meta learning, and \citet{maggipinto2020proximal} improved TD3~\citep{td3} by employing a stochastic proximal-point interpretation.

The effect of the proximal term in our work is reminiscent of the use of trust regions in policy-gradient algorithms~\citep{trpo,ppo, YuhuiNEURIPS2019, fakoor2019p3o, tomar2021mirror}. However, three factors differentiate our work: we define the proximal term using the value function, not the policy, we enforce the proximal term in the parameter space, as opposed to the function space, and we use the target network as the previous iterate in our proximal definition. 

%Finally, existing work showed the benefits of leveraging the structure of the RL problem during optimization. \citet{precup1997exponentiated} argued that the space of value functions could better be understood as a manifold with an entropic metric. \citet{mahadevan2012sparse} used mirror descent to penalize weights with large p-norms. Similarly, \citet{van2019using} advocated for performing Q-updates in a logarithmic space to combat issues that arise due to the action-gap phenomena~\citep{farahmand2011action}.



==> PI for Deep Reinforcement Learning (Neurips 2022)/theory.tex <==
\section{Proximal Bellman Operator}
In this section, we introduce a new class of Bellman operators that ensure that the next iterate in planning and RL remain in the vicinity of the previous iterate. To this end, we define the Bregman Divergence generated by a convex function $f$:
$$
D_{f}(v',v) \myeq f(v') - f(v) - \langle \nabla f(v), v'-v \rangle\ .
$$
Examples include the $l_{p}$ norm generated by $f(v)=\frac{1}{2}\norm{v}{p}{2}$ and the Mahalanobis Distance generated by $f(v)=\frac{1}{2}\langle v,Q v \rangle$ for a positive semi-definite matrix $Q$.

We now define the Proximal Bellman Operator $(\mathcal{T}^{\pi}_{c, f})^n$:
\begin{equation}
    (\mathcal{T}^{\pi}_{c, f})^n v \myeq\arg\min_{v'} ||v'- (\mathcal{T}^{\pi})^n v||^{2}_{2} +\frac{1}{c} D_{f}(v',v)\ ,
    \label{eq:proximal_bellman_operator}
\end{equation}

where $c\in(0,\infty)$. Intuitively, this operator encourages the next iterate to be in the proximity of the previous iterate, while also having a small difference relative to the point recommended by the original Bellman Operator. The parameter $c$ could, therefore, be thought of as a knob that controls the degree of gravitation towards the previous iterate.

Our goal is to understand the behavior of Proximal Bellman Operator when used in conjunction with the Modified Policy Iteration (MPI) algorithm~\citep{PutermanMDP1994, ampi}. Define $\mathcal{G}v$ as the greedy policy with respect to $v$.
% zzz MLL: define, for completeness?
At a certain iteration $k$, Proximal Modified Policy Iteration (PMPI) proceeds as follows:
\begin{eqnarray}
\pi_{k} &\leftarrow& \mathcal{G} v_{k-1}\ \label{eq:pmpi_1} ,\\
v_{k} &\leftarrow& (\mathcal{T}^{\pi_{k}}_{c, f})^{n} v_{k-1} \label{eq:pmpi_2}\ .
\end{eqnarray}
The pair of updates above generalize existing algorithms. Notably, with $c\rightarrow\infty$ and general $n$ we get MPI, with $c\rightarrow\infty$ and $n=1$ the algorithm reduces to Value Iteration, and with $c\rightarrow\infty$ and $n=\infty$ we have a reduction to Policy Iteration. For finite $c$, the two extremes of $n$, namely $n=1$ and $n=\infty$, could be thought of as the proximal versions of Value Iteration and Policy Iteration, respectively.

To analyze this approach,
it is first natural to ask if each iteration of PMPI could be thought of as a contraction so we can get sound and convergent behavior in planning and learning. For $n> 1$, \citet{ampi} constructed a contrived MDP demonstrating that one iteration of MPI can unfortunately expand. As PMPI is just a generalization of MPI, the same example from \citet{ampi} shows that PMPI can expand. In the case of $n=1$, we can rewrite the pair of equations (\ref{eq:pmpi_1}) and (\ref{eq:pmpi_2}) in a single update as follows:
$v_k \leftarrow \mathcal{T}^{\star}_{c, f} v_{k-1}\ .$
When $c\rightarrow\infty$, standard proofs can be employed to show that the operator is a contraction~\citep{littman_csaba}.
We now show that $\mathcal{T}^{\star}_{c, f}$ is a contraction for finite values of $c$. See our appendix for proofs.
\begin{restatable}[]{thm}{contraction}
\label{thm:goldbach}
The Proximal Bellman Optimality Operator $\mathcal{T}^{\star}_{c, f}$ is a contraction with fixed point $v^{\star}$.
\end{restatable}
Therefore, we get convergent behavior when using $\mathcal{T}^{\star}_{c, f}$ in planning and RL. The addition of the proximal term is fortunately not changing the fixed point, thus not negatively affecting the final solution.
This could be thought of as a form of regularization that vanishes in the limit; the algorithm converges to $v^{\star}$ even without decaying $1/c$.

% zzz ML: What follows is hard to follow. Terms like Euclidean norm and estimate of the Bellman operator and evaluation step aren't spelled out at the pace used before this page. Also, "interested in understanding" is not providing a lot of guidance about what is coming next. You already explained that MPI isn't a non-expansion. So, what's left to say??
% I strongly think we should lead off with the punchline and how we plan to support it. (Are we giving the full argument, or a sketch in a simplified setting?) Then provide some math as shown. (Although, putting it in the appendix seems fine to me.)
Going back to the general $n\geq 1$ case, we cannot show contraction, but following previous work~\citep{bertsekas1996neuro, ampi}, we study error propagation in PMPI in presence of additive noise where we get a noisy sample of the original Bellman Operator $(\mathcal{T}^{\pi_k})^n v_{k-1}+\epsilon_{k}$. The noise can stem from a variety of reasons, such as approximation or estimation error. For simplicity, we restrict the analysis to $D_f(v',v)= ||v'-v||^{2}_{2}$, so we rewrite update (\ref{eq:pmpi_2}) as:
$$v_{k}\leftarrow \arg\min_{v'} ||v'- \big((\mathcal{T}^{\pi_k})^n v_{k-1}+\epsilon_{k}\big)||^{2}_{2} +\frac{1}{c} \norm{v'-v_{k-1}}{2}{2}$$
which can further be simplified to:
$$v_{k}\leftarrow \underbrace{(1-\beta)(\mathcal T^{\pi_k})^{n}v_{k-1}+ \beta v_{k-1}}_{:=(\mathcal{T}^{\pi_k}_{\beta})^n v_{k-1}} +(1-\beta)\epsilon_{k} , $$
where $\beta=\frac{1}{1+c}$. This operator is a generalization of the operator proposed by~\citet{smirnova2020convergence} who focused on the case of $n=1$. To build some intuition, notice that the update is multiplying error $\epsilon_k$ by a term that is smaller than one, thus better hedging against large noise. While the update may slow progress when there is no noise, it is entirely conceivable that for large enough values of $\epsilon_k$, it is better to use non-zero $\beta$ values. In the following theorem we formalize this intuition. Our result leans on the theory provided by \citet{ampi} and could be thought of as a generalization of their theorem for non-zero $\beta$ values.

\begin{restatable}[]{thm}{error}
\label{thm:loss_bound}
Consider the PMPI algorithm specified by:
\begin{eqnarray}
\pi_{k} &\leftarrow& \mathcal{G}_{\epsilon'_k} v_{k-1}\ ,\\
v_{k}&\leftarrow& (\mathcal{T}^{\pi_k}_{\beta})^n v_{k-1} +(1-\beta)\epsilon_k\ .
\end{eqnarray}


Define the Bellman residual $b_k\myeq v_{k} - \mathcal{T}^{\pi_{k+1}}v_k$, and error terms $x_k := (I-\gamma P^{\pi_{k}})\epsilon_k$ and $y_k:=\gamma P^{\pi^*}\epsilon_{k}$.
After $k$ steps:
$$ v^{*} - v^{\pi_k} = \underbrace{v^{\pi^{*}}-(\mathcal{T}^{\pi_{k+1}}_{\beta})^n v_k}_{d_k} +\underbrace{(\mathcal{T}^{\pi_{k+1}}_{\beta})^n v_k - v_{\pi_k}}_{s_k} $$
\begin{itemize}
    \item where $d_{k} \leq \gamma P^{\pi^{*}}d_{k-1} -\big((1-\beta)y_{k-1} + \beta b_{k-1}\big) + (1-\beta)\sum_{j=1}^{n-1}(\gamma P^{\pi_{k}})^j b_{k-1} + \epsilon'_{k}$
    \item $s_k \leq \big((1-\beta)(\gamma P^{\pi_k})^n + \beta I\big)(I-\gamma P^{\pi_k})^{-1}b_{k-1}$
    \item $b_{k} \leq \big((1-\beta)(\gamma P^{\pi_k})^{n} + \beta I\big) b_{k-1}+ (1-\beta) x_{k} + \epsilon'_{k+1}$
\end{itemize}
\end{restatable}

The bound provides intuition as to how the proximal Bellman Operator can accelerate convergence in the presence of high noise. For simplicity, we will only analyze the effect of the $\epsilon$ noise term, and ignore the $\epsilon'$ term. We first look at the Bellman residual, $b_k$. Given the Bellman residual in iteration $k-1$, $b_{k-1}$, the only influence of the noise term $\epsilon_k$ on $b_k$ is through the $(1-\beta) x_k$, term, and we see that $b_k$ decreases linearly with larger $\beta$.

The analysis of $s_k$ is slightly more involved but follows similar logic. The bound for $s_k$ can be decomposed into a term proportional to $b_{k-1}$ and a term proportional to $\beta b_{k-1}$, where both are multiplied with positive semi-definite matrices. Since $b_{k-1}$ itself linearly decreases with $\beta$, we conclude that larger $\beta$ decreases the bound quadratically.

The effect of $\beta$ on the bound for $d_k$ is more complex. The terms $\beta y_{k-1}$ and $\sum_{j=1}^{n-1}(\gamma P^{\pi_{k}})^j b_{k-1}$ introduce a linear decrease of the bound on $d_k$ with $\beta$, while the term $\beta (I - \sum_{j=1}^{n-1}(\gamma P^{\pi_{k}})^j) b_{k-1}$ introduces a quadratic dependence whose curvature depends on $I - \sum_{j=1}^{n-1}(\gamma P_{\pi_{k}})^j$. This complex dependence on $\beta$ highlights the trade-off between noise reduction and magnitude of updates. To understand this trade-off better, we examine two extreme cases for the magnitude on the noise. When the noise is very large, we may set $\beta=1$, equivalent to an infinitely strong proximal term. It is easy to see that for $\beta=1$, the values of $d_k$ and $s_k$ remain unchanged, which is preferable to the increase they would suffer in the presence of very large noise. On the other extreme, when no noise is present, the $x_k$ and $y_k$ terms in Theorem~\ref{thm:loss_bound} vanish, and the bounds on $d_k$ and $s_k$ can be minimized by setting $\beta=0$, i.e. without noise the proximal term should not be used and the original Bellman update performed. Intermediate noise magnitudes thus require a value of $\beta$ that balances the noise reduction and update size.
% zzz MLL: I'm left feeling like there's a gap here. Why do we care about additive noise? Is it standing in for something else? If so, is there a relationship (even empirically) between what we really care about (bias introduced by function approximation? uncertainty due to sampling?) and the proximal approach? I'd like to see a plot from a realistic problem showing the optimal value of beta (but can we even control beta? I thought it was c.) for a range of something (stochasticity in the test environment, like slip probability in a grid, say?).

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}
\usepackage{mathtools}
% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> proximal_bellman_operator.tex <==
\section{The Proximal Bellman Equation}
Define 

$$T_{\proxNoParanthesis{h}}(Q):=\proxNoParanthesis{h}\big(T(Q)\big).$$
We show that $Q^{*}$, defined as the fixed point of the original Bellman equation, $Q^{*}=TQ^{*}$ is also the fixed point of the proximal Bellman equation:
$$Q^{*}=\proxNoParanthesis{h}\big(T(Q^*)\big)\ ,$$
under zzz condition on $h$. This result demonstrates that, while adding the proximal term biases the interim solution towards those with small $h$, this bias will vanish as we converge to the fixed-point solution in light of the equivalence between the fixed points of $T$ and $T_{\proxNoParanthesis{h}}$. We prove this statement in the following Theorem:

\begin{theorem}
\label{thm:convergence_general}
Let $\mathcal{O}:\mathcal{V} \rightarrow \mathcal{V}$ be a contraction operating on the vector space $\mathcal{V}$. Let
\begin{align}
    \prox{f,V'}{V} \equiv \argmin_{\hat{V}} \left[ f(V, \hat{V}) + \norm{\hat{V} - V'}{2}{2} \right]
\end{align}

\textcolor{red}{$$ 
    \prox{f,V'}{V} \equiv \argmin_{\hat{V}} \left[ f(V', \hat{V}) + \norm{\hat{V} - V}{2}{2} \right]$$}
% \begin{align}
%     \prox{f,V'}{V} \equiv \argmin_{\hat{V}} \left[ f(\hat{V}, \hat{V}) + \norm{\hat{V} - V}{2}{2} \right]
% \end{align}

with $f:\mathcal{V} \times \mathcal{V} \rightarrow \mathbb{R}$ a convex function such that $\argmin_V f(V, V') = V'$. Then, the sequence $V_k$ given by

\begin{align}
    V_{k+1} = \prox{f,\mathcal{O}(V_k)}{\mathcal{O}(V_k)}
\end{align}

and any $V_0 \in \mathcal{V}$ converges to the fixed point of $\mathcal{O}$, denoted as $V^*$.

\end{theorem}

\begin{proof}
Define the operator

\begin{align}
    \mathcal{O}_{\textbf{prox}_{f,V'}}(V) = \prox{f,V'}{\mathcal{O}(V)} = (\textbf{prox}_{f,V'} \circ \mathcal{O}) (V).
\end{align}
Then, we can write the sequence $V_k$ as $V_{k+1} = (\textbf{prox}_{f,V_k} \circ \mathcal{O}) (V_k)$. Because the proximal operator is a non-expansion, and $\mathcal{O}$ is a contraction, the composition $\textbf{prox}_{f,V_k} \circ \mathcal{O}$ is also a contraction and therefore has a unique fixed point. We must therefore only show that $V^*$ is a fixed point of
\begin{align}
    \prox{f,V^*}{V} \equiv \argmin_{\hat{V}} \left[ f(V, \hat{V}) + \norm{\hat{V} - V^*}{2}{2} \right].
\end{align}

\textcolor{red}{$$ \prox{f,V^*}{V} \equiv \argmin_{\hat{V}} \left[ f(V^*, \hat{V}) + \norm{\hat{V} - V}{2}{2} \right]
$$}

\textcolor{red}{$$ = \argmin_{\hat{V}} \left[ f(V^*, \hat{V}) + \norm{\hat{V} - V}{2}{2} \right]
$$}

% \begin{align}
%     \prox{f,V^*}{V} \equiv \argmin_{\hat{V}} \left[ f(V, V^*) + \norm{\hat{V} - V}{2}{2} \right].
% \end{align}

But $V^*$ eliminates the second term and, by our assumption on $f(V)$, minimizes the first term. Therefore, $\prox{f,V^*}{V^*} = V^*$.

\end{proof}

Note that Theorem \ref{thm:convergence_general} is much more general and extends beyond applying an $L_2$ norm to the Bellman operator. It shows that the adding a proximal step can be applied to many RL operators without biasing the fixed point these algorithms converge to. Thus, for example, when applying the proximal step to linear function approximation of the Bellman operator {\bf a reference would be good}, we would still converge to the same projected fixed point of the Bellman operator onto the linear space, because projections maintain the contraction properties of operators. Furthermore, $f(V)$ does not necessarily have to be the $L_2$ norm (and doesn't even have to be a norm), opening the door to a variety of potential algorithms using different convex regularization functions. % zzz MLL: I'd move the more abstract Lemma 2 into supplementary material since the proof is SO similar to the first one and is mainly here for flag planting, it seems.

Notation-wise, we have

$$T_{\proxNoParanthesis{h}}(Q):=\proxNoParanthesis{h(\cdot;Q)}(Q)$$
i.e. when the argument of T and the second argument of $h$ are the same, we just drop it from $h$ for readability. also please always use $h$ as the letter that indicates a generic proximal function.

% We first show that the operator $T_{\prox{f}{V}}$ converges to the same fixed point as $T$, that is, both converge to the optimal value function $V^*$.

% \begin{lemma}
% \label{lemma:simple_convergence}
%     The operator $T_{\prox{f}{V}}$ is a contraction, with the same fixed point, $V^*$, as the Bellman operator, $T$. 
% \end{lemma}

% \begin{proof}
% The $T_{\prox{f}{V}}$ is a composition of the Bellman operator and the proximal operator. Because the Bellman operator is a contraction (CITE) and the proximal operator is a non-expansion \citep{beck_book}, their composition is also a contraction, and therefore has a unique fixed point. We therefore only need to show that $V^*$, the fixed point of $T$, is also a fixed point of $T_{\prox{f}{V}}$.

% At $V^*$, $T_{\prox{f}{V}}$ can be explicitly written as:

% \begin{align*}
%     T_{\prox{f}{V^*}}(V) \equiv \argmin_{\hat{V}} \left[ \norm{TV - \hat{V}}{2}{2} + \norm{V^*-\hat{V}}{2}{2} \right].
% \end{align*}

% % MLL: I'd make this point differently.
% Setting $\hat{V} = V^*$, makes the second term zero and also makes the first term zero because $V^*$ is a fixed point of $T$. The entire expression is necessarily non-negative, making $V^*$ a minimizer. Thus, $T_{\prox{f}{V^*}}(V^*) = V^*$; $V^*$ is a fixed point.

% % For $\hat{V} = V^*$, the first term vanishes because $V^*$ is a fixed point of T, and the second term vanishes trivially. The entire expression to be minimized by the operator is non-negative, and therefore minimized by $V^*$. Thus $T_{\prox{f}{V^*}}(V^*) = V^*$

% \end{proof}


==> proximal_operator.tex <==
\section{Proximal Operator [TODO merge ]}
\label{sec:proximal_operator}
Consider the following optimization problem:
\begin{equation}
    %\arg\min_w h(w)\ ,
    \min_w ~h(x;w)\ ,
    \label{eq:original_problem}
\end{equation}
%where $h$ could be any objective function such as a loss function for learning the Q-function in reinforcement learning, and $w$ denotes the parameters of the network we desire to learn. Suppose we have access to stochastic estimates of the gradient of the function $\nabla h$. Standard first-order optimization, such as stochastic gradient descent (SGD), can be employed to solve this optimization problem:
where $h$ is the objective function (e.g., standard temporal difference (TD) error in reinforcement learning~\ref{eq:td_error}), $w$ denotes the learnable parameters (e.g., the parameters of a Q-network), and $x$ is the input data (e.g., $\langle s, a, r, s' \rangle$). If $h$ is differentiable, then stochastic gradient descent (SGD), which proceeds as follows:
%$$w_{k+1}\leftarrow w_{k} -\alpha_{k} \nabla h(w_k)\ ,$$
\begin{equation}\label{eq:sgd}
w_{k}\leftarrow w_{k-1} -\alpha_{k} \nabla_w h(x;w_{k-1}), ~~~k=1,2,3,\dots
\end{equation}
could be used to solve the optimization problem~(\ref{eq:original_problem}). Here, $\alpha_k$ denotes the step size at iteration $k$, and $w_0$ is an arbitrary starting point.

While SGD is well-behaved asymptotically and under standard assumptions, it can perform recklessly in the interim, leading into a situation where the iterates get exponentially far from the %optimal
solution~\citep{BachNIPS2011, ryu_boyd_proximal}. This behavior can be particularly disruptive in the context of RL where sample efficiency is an important concern.

One simple and effective approach to stabilizing SGD is to augment the objective with a quadratic regularizer to ensure that the solution at each iteration stays in the vicinity of the previous ones:
%. This can be obtained by augmenting the objective as follows:
\begin{equation}
    w_{k} = \arg\min_w h(w) + \frac{1}{2c}\norm{w-w_{k-1}}{2}{2}\ .
    \label{eq:modified_problem}
\end{equation}
The quadratic term is basically a proximal term that ensures the next iterate $w_k$ will not stray too far from the previous iterate $w_{k-1}$. Having completed iteration $k$, we replace the previous iterate $w_{k-1}$ by its new value $w_k$ and then proceed to iteration $k+1$.
\iffalse 
To understand the behavior of this iterative process, called Proximal Iteration~\citep{prox_parikh_boyd, ryu_boyd_proximal}, we define the proximal operator:
\begin{equation}
    \prox{c, h}{w_k}:=\arg\min_{w}\ \frac{1}{c}\norm{w-w_{k-1}}{2}{2} +\ h(w)\ ,
\end{equation}
Proximal Iteration could be written as:
$$
w_{k}\leftarrow \prox{h}{w_{k-1}}\ ~~~k=1, 2, 3\dots
$$
From the Banach fixed-point theorem, we know that iteratively applying $\proxNoParanthesis{h}$ eventually converges to a unique fixed point provided that the operator is a contraction. \cite{bauschke2012firmly} have shown that, if the function $h$ is $\mu$-strongly convex, then the operator $\proxNoParanthesis{h}$ is indeed a contraction:
$$\norm{\prox{h}{w}-\prox{h}{w'}}{}{}\leq \frac{1}{1+\mu}\norm{w-w'}{}{}\ ,$$
and therefore iteratively applying the operator would guarantee convergence. 

What is the fixed-point of this operator? It is possible to show that it is the minimum of the function $h$, i.e., $\arg\min_{w} h(w)$, the minimum of problem~(\ref{eq:original_problem}), which we originally sought to solve~\citep{bauschke2011convex}. 

Therefore, the intuitive way of thinking about the Proximal Iteration algorithm, which is sometimes referred to as disappearing Tikhonov regularization~\citep{prox_parikh_boyd}, is as a principled way to bias the optimization path towards the previous iterate using the quadratic-norm penalty without altering the final answer. In other words, as Proximal Iteration makes progress, the previous iterate $w_{k-1}$ gets closer to $w^{\star}=\arg \min h(w)$ in light of the contraction property, therefore the contribution of the quadratic term vanishes to zero thus not biasing the asymptotic solution. The following remark sheds more light on the relationship between Proximal Iteration and trust-region algorithms:

[\textbf{Relationship between trust region and Proximal Iteration}]\label{rem:trust-region}
Define the trust-region problem as follows:
\begin{align*}\label{eq:trust_problem}
    %&\arg\min_w ~h(w)\\
    & \displaystyle{\min}_w ~h(w)\\
    &\text{s.t.}\ \norm{w-w_{k-1}}{2}{} \leq \rho\ , 
\end{align*}
\cite{prox_parikh_boyd} show that solving the above trust-region formulation is equivalent to a step of Proximal Iteration under appropriate choices of  $\rho$ (above) and $c$ (in prox). Therefore, iteratively applying the two formulations leads to the same solution. (See their Section~3.4 for more details.) %This interpretation provides \
%\todo[ "trust region formulation is equivalent to a step of Proximal" is not what they showed and I don't think so "a step of Proximal Iteration" is their result. they clearly showed proximal and trust region both get to the same solution with some combination of their hyper-params.... What I originally wrote provided a right version for their results: \cite{prox_parikh_boyd} shows that above trust region formulation and proximal problem~\eqqref{eq:modified_problem} are related and both methods can get to the same solutions for appropriate choices of their parameters (i.e $\rho$, $c$ ) (see section 3.4 in their paper for more details). Kavosh: one step of proximal iteration = one step of trust region, do both multiple times and you get the same answer.]
The second remark highlights the strength of Proximal Iteration relative to SGD:
[\textbf{The non-asymptotic advantage of Proximal Iteration over SGD}]\label{rem:non-asymptotic}
\fi
While the asymptotic performance of SGD and Proximal Iteration are analogous~\citep{ryu_boyd_proximal}, they may exhibit qualitatively different behavior in a non-asymptotic sense. More concretely, denote the stepsize of SGD and Proximal Iteration at iteration $k$ by $\alpha_k=\frac{C}{k}$, and $w^{\star}:=\arg\min_w h(w)$. For SGD, we have~\citep{bauschke2011convex}:
$$\expectation{}\big[\norm{w_k-w^{\star}}{2}{2}\big]\leq \mathcal{O}\left(\frac{\textrm{exp}(C^{2})}{k^{ C}} + \frac{1}{k}\right)\ .$$
The exponential dependence on $C$ can indeed manifest itself as \cite{ryu_boyd_proximal} demonstrate. In contrast, for Proximal Iteration we have~\citep{ryu_boyd_proximal}:
$$\expectation{}\big[\norm{w_k-w^{\star}}{2}{2}\big]\leq \norm{w_0-w^{\star}}{2}{2} +\sum_{i=1}^k \alpha_i\ .$$
While the iterates of SGD can get exponentially far from the optimal answer~\citep{BachNIPS2011, ryu_boyd_proximal}, Proximal Iteration is fairly well-behaved in the interim. This property is particularly valuable in the context of reinforcement learning where sample-efficiency, and not just the asymptotic performance, is of utmost importance.

\iffalse
In the context of a parameterized $Q$-function in RL, commonly used loss functions are not convex; however, several works have introduced convex loss via linear approximation. \citet{target_based_TD} have shown that in linear policy evaluation the loss function is convex in the weights. \citet{serrano2021logistic} introduced a convex loss function for control with linear approximation. These works demonstrate that many useful convex minimization objectives exist for RL.

In the case of deep RL, the loss function is not convex, and few convergence results exist for most state-of-the-art algorithms. Nevertheless, we follow standard practice and show that Proximal Iteration achieves significant empirical improvements when applied to standard deep RL algorithms. Furthermore, recent work provides convergence results for Proximal Iteration in specific non-convex cases, such as when $h(w)$ can be decomposed into a sum of a smooth non-convex function and non-smooth convex function~\citep{fukushima1981generalized, j2016proximal, li2018simple}. These recent results open the door for potential future developments toward proving convergence for Proximal Iterations in RL, which would further strengthen its theoretical grounding.
\fi
